Behaviorally Correct Learning from Informants

In inductive inference, we investigate the learnability of classes of formal languages. We are interested in what classes of languages are learnable in certain learning settings. A class of languages is learnable, if there is a learner that can identify all of its languages and satisfies the constraints of the learning setting. To identify a language, a learner is presented with information about this very language. When learning from informants, this information consists of examples for numbers that are, and numbers that are not included in the target language. As more and more examples are presented, the learner outputs a hypothesis sequence. To satisfy behaviorally correct identification, this hypothesis sequence must eventually only list correct labels for the target language. In this thesis, we compare the effects of a number of semantic learning restrictions on the learning capabilities for behaviorally correct learning from informants.

==> core/purgatory.tex <==
\begin{theorem}
    We have $[\Inf\G\Bc] = [\Inf\Sd\Bc]$.
\end{theorem}
\begin{proof}
    Obviously, $[\Inf\Sd\Bc] \subseteq [\Inf\G\Bc]$, so it suffices to show that $[\Inf\G\Bc] \subseteq [\Inf\Sd\Bc]$.
    Let $\La$ be a set of languages that is $\Inf\G\Bc$-learnable and let $h$ be such a learner.
    We construct an $\Sd$ learner $h'$ that will return the prediction of $h$ given the longest possible prefix of a canonical informant that $h'$ can construct from the information it has.

    We define the length of the built prefix
    $$l: X \mapsto \max\set{n \in \N \with \forall i < n: i \in \outline(X)}$$
    the information about each element
    $$c: X \mapsto ((i, \indic{\pos(X)}{(i)}))_{i < l(X)}$$
    the canonical prefix and lastly, the learner
    $$h' = h \circ c.$$
    Notably, for any $\sigma$ and $n \in \N$ with $\set{0, 1, \dots, n} \subseteq \outline(\sigma)$, we have $\hat I_P[n] \sqsubseteq c(\content(\sigma))$.
    It can easily be argued that all of the above are computable functions.

    Let $L \in \La$. There is $\hat n \in \N$ such that for all $n \geq \hat n$ we have $W_{h(\hat I_L[n])} = L$.
    Let $I \in \Inf(L)$ and $n_0 \geq \hat n$ with $\set{0, 1, \dots, \hat n} \subseteq \outline(I[n])$.
    Thus, for all $n \geq n_0$ we have $l(\content(I[n])) \geq \hat n$ and
    $\hat I_L[\hat n] \sqsubseteq c(\content(I[n])) \sqsubseteq \hat I_L[n]$.
    Hence, $$W_{h'(\content(I[n]))} = W_{h(c(\content(I[n])))} = W_{h(\hat I_L[\hat n])} = L.$$
\end{proof}

\begin{theorem}
    We have $[\Inf\G\Cons\WMon\Bc] = [\Inf\G\WMon\Bc]$.
\end{theorem}
\begin{proof}
    Let $h$ be a $\G$-learner and $\La = \Inf\G\WMon\Bc(h)$.
    By \Cref{thm:totalInteractionForDelayable}, as $\WMon\Bc$ is delayable, we can assume $h$ to be total.
    Consider the $\G$-learner $g$ that maps a finite sequence $\sigma \in \Seq(\N \times \bset)$ to the hypothesis
    \begin{align*}
        W_{g'(\sigma)} &= \begin{cases}
            \N \setminus \neg(\sigma), &\text{if } \exists \tau \subsetneq \sigma: \neg(\tau) = \neg(\sigma) \land W_{g(\tau)} = \N \setminus \neg(\sigma), \\
            \pos(\sigma),              &\text{else if } \pos(\sigma) \not\subseteq W_{h(\sigma)}, \\
            W_{h(\sigma)},             &\text{else if } \Cons(h(\sigma), \sigma), \\
            \N \setminus \neg(\sigma), &\text{otherwise}.
        \end{cases}\\
        g(\sigma) &= g'\left( \argmin_{\tau \subseteq \sigma, \content(\tau) = \content(\sigma)} \cardinality \tau \right).
    \end{align*}

    To enumerate $W_{g(\sigma)}$, the program $g(\sigma)$ would do the following:
    Given some input $x \in \N$, if $x \in \pos(\sigma)$, it returns, if $x \in \neg(\sigma)$, it diverges.
    Then, it verifies that $\pos(\sigma) \subseteq W_{h(\sigma)}$, diverging if this is not the case.
    Finally, it searches for either of the following cases:
    \begin{itemize}
        \item verifying $x \in W_{h(\sigma)}$,
        \item finding some $y \in \neg(\sigma) \cap W_{h(\sigma)}$ or
        \item finding some $\tau \subsetneq \sigma$ with $\neg(\tau) = \neg(\sigma)$, $\pos(\tau) \subseteq W_{h(\tau)}$ and $\exists y \in \neg(\sigma) \cap W_{h(\tau)}$.
    \end{itemize}

    Clearly, $g$ is consistent.
    Let $L \in \La$ and $I \in \Inf(L)$.
    Let $n_0 \in \N$ be such that for all $n \geq n_0$ we have $W_{h(I[n])} = L$.
    If $\overline L$ is finite, let $n_1 \geq n_0$ be such that $\neg(I[n_1]) = \overline L$.
    Then, we have for all $n \geq n_1$ that $W_{g(I[n])} = L$, because the second case of $g$ is false for $n$ and all other cases output $L$.
    Suppose that $\overline L$ is infinite.
    Let $n_2 \in \N$ be minimal with $n_2 > n_0$ and $\neg(I[n_0]) \subsetneq \neg(I[n_2])$.
    By induction, we get for all $n \geq n_2$ that the first two cases of $g$ are false for input $I[n]$ and thus $W_{g(n)} = W_{h(n)} = L$.

    We proceed to show that $g$ is weakly monotonic.
    Let $s, t \in \N$ with $s < t$.
    We abbreviate $S = I[s]$ and $T = I[t]$.
    Suppose $\Cons(g(S), T)$.

    \paragraph{Case 1: $W_{g(S)} = \pos(S)$.}
    By the consistency of $g$ we have $W_{g(S)} = \pos(S) \subseteq \pos(T) \subseteq W_{g(T)}$.
    \paragraph{Case 2: $W_{g(S)} = W_{h(S)}$.}
    This implies $\Cons(h(S), T)$ and by $h$ being weakly monotonic, $W_{h(S)} \subseteq W_{h(T)}$.
    Since $\pos(T) \subseteq W_{h(S)} \subseteq W_{h(T)}$, $g(T)$ cannot be the second case.
    As we have $W_{h(S)} \subseteq W_{h(T)}$ and $W_{h(S)} \subseteq \N \setminus \neg(T)$, weak monotonicity is fulfilled.
    \paragraph{Case 3: $W_{g(S)} = \N \setminus \neg(S)$.}
    As $\Cons(g(S), T)$, we must have $\neg(S) = \neg(T)$.
    Then, with $\tau = S$, $g(T)$ uses the first case and we have $W_{g(S)} = W_{g(T)}$.
\end{proof}

